Do Noises Bother Human and Neural Networks In the Same Way? A Medical Image Analysis Perspective

Deep learning had already demonstrated its power in medical images, including denoising, classification, segmentation, etc. All these applications are proposed to automatically analyze medical images beforehand, which brings more information to radiologists during clinical assessment for accuracy improvement. Recently, many medical denoising methods had shown their significant artifact reduction result and noise removal both quantitatively and qualitatively. However, those existing methods are developed around human-vision, i.e., they are designed to minimize the noise effect that can be perceived by human eyes. In this paper, we introduce an application-guided denoising framework, which focuses on denoising for the following neural networks. In our experiments, we apply the proposed framework to different datasets, models, and use cases. Experimental results show that our proposed framework can achieve a better result than human-vision denoising network.

==> Section/Related_Works.tex <==
In this section, we introduce several existed works for medical image denoising, segmentation, and classification.

\subsection{Medical Image Denoising}

In the past few years, lots of denoising methods were proposed to produce clean image on various types of image. In this paper, we limit the discussion into medical image such as CT and MRI to demonstrate the efficacy of our method in the experiment.

For CT, Wolterink et al. \cite{wolterink2017generative} designed a generative adversarial network (GAN) denoising model with Convolution Neural Network (CNN) as generator, which tried to keep the reality for the denoised output. Yang et al. \cite{yang2018low} adopted Wasserstein distance and perceptual loss to ensure the similarity between input and the generated image.
For MRI, Manj{\'o}n and Coupe \cite{manjon2018mri} proposed a simple CNN network for 2D MRI artifact reduction. Li et al. \cite{li2019two} then proposed a two-stage reconstruct network to generate super resolution MRI.

As clean images are usually expensive to obtain, all these methods mentioned require simulations or synthesis for dataset. Moreover, they focused on how denoising affected human eyes, which tried to reduce every noise contained inside images. Using such loss function as mean square error (MSE) or structural similarity index (SSIM), they could minimize the difference between generated output and the ground-truth. Although they achieve superior performance and results for human vision, when it comes to machine vision scenario they might not be the most suitable solution. Thus, we proposed the framework which utilizes the application loss to optimize the denoising network.

\subsection{Medical Image Segmentation}

Segmentation for medical image has been popular for a few years, it segments the input image into several regions of different categories. As playing such an important role in automatic disease diagnosis, it provides fast speed assessment and more valuable information for radiologists. For example, a segmentation method could automatically discover brain tumor in early step, which reduces efforts made by doctors.

As many medical image segmentation methods have been proposed in the literature, U-Net \cite{ronneberger2015u} based methods are the most popular network structure for biomedical segmentation. Ronneberger et al. \cite{ronneberger2015u} proposed the fundamental U-Net structure for 2D biomedical segmentation. Isensee et al. \cite{isensee2018no} then applied U-Net into 3D brain tumor CT segmentation with minor modifications. Christ et al. \cite{christ2016automatic} combined U-Net model and Fully Convolutional Neural Network (FCN) to 3D CT image segmentation for liver and lesion.

\subsection{Medical Image Classification}

Classification is considered as a similar problem with segmentation. It aims to figure out which category does the full input image fell into, which brings many benefits for automatic diagnosis. Among all existed medical image classification, Convolution Neural Network (CNN) based structure is still the most common network architecture. Li et al. \cite{li2014medical} applied CNN to 2D CT image classification at interstitial lung disease classification task. Shen et al. \cite{shen2015multi} and Kumar et al. \cite{kumar2015lung} introduced 3D CNN and autoencoder, respectively, for lung nodule classification in CT image. Sultan et al. \cite{sultan2019multi} then designed another CNN model for brain tumor classification in MRI image.

